Best Arm Identification with Fixed Budget: A Large Deviation Perspective

We consider the problem of identifying the best arm in stochastic Multi-Armed Bandits (MABs) using a fixed sampling budget. Characterizing the minimal instance-specific error probability for this problem constitutes one of the important remaining open problems in MABs. When arms are selected using a static sampling strategy, the error probability decays exponentially with the number of samples at a rate that can be explicitly derived via Large Deviation techniques. Analyzing the performance of algorithms with adaptive sampling strategies is however much more challenging. In this paper, we establish a connection between the Large Deviation Principle (LDP) satisfied by the empirical proportions of arm draws and that satisfied by the empirical arm rewards. This connection holds for any adaptive algorithm, and is leveraged (i) to improve error probability upper bounds of some existing algorithms, such as the celebrated \sr (Successive Rejects) algorithm \citep{audibert2010best}, and (ii) to devise and analyze new algorithms. In particular, we present \sred (Continuous Rejects), a truly adaptive algorithm that can reject arms in {\it any} round based on the observed empirical gaps between the rewards of various arms. Applying our Large Deviation results, we prove that \sred enjoys better performance guarantees than existing algorithms, including \sr. Extensive numerical experiments confirm this observation.

==> sec/4.algorithmOLD.tex <==
\section{Continuous Rejects Algorithms}\label{sec:cr}

In this section, we present \sred, a truly adaptive algorithm that can discard an arm in {\it any} round. We propose two variants of the algorithm, \crc using a conservative criterion to discard arms and \cra discarding arms more aggressively. Using the Large Deviaition results of Theorem \ref{thm:Varadaham bandits}, we establish error probability upper bounds for both \crc and \cra. 


%\cite{audibert2010best}, many works have pointed out the lack of adaptiveness in \sr, which may waste too much budget for pulling an empirical poor arm before the phase ends. \sred, in contrast, discard an arm at any round once the condition of discard is met. There are two variants, the one discarding conservatively is called \crc, and the other doing aggressively is called \cra. These algorithms will be explicitly presented below. Under an additional assumption that $\bm\in [0,1]^K$, their analysis in Theorem \ref{thm:crc} and \ref{thm:cra} in \textsection \ref{sec:anal cr}.     

\subsection{The \crc and \cra algorithms}

As \sr, \sred initializes its candidate set as $\mathcal{C}_K=[K]$. For $j\ge 2$, ${\cal C}_j$ denotes the candidate set when it is reduced to $j$ arms. When $j>2$, the algorithm samples arms in the candidate set ${\cal C}_j$ uniformly until a {\it discarding condition} is met. The algorithm then discards the empirically worst arm $\ell_j\in {\cal C}_j$, i.e., $\mathcal{C}_{j-1}\leftarrow \mathcal{C}_j\setminus \{\ell_j\}$. More precisely, in round $t$, if there are $j$ candidate arms remaining and if $\ell(t)$ denotes the empirically worst candidate arm, the discarding condition is $N_{\ell(t)}(t)>\max_{k\notin \mathcal{C}_j}N_k(t),\, (\forall k\in \mathcal{C}_j,\,N_{\ell(t)}(t)=N_{k}(t))$\footnote{This condition is only imposed to simplify our analysis. It may be removed.}, and
\begin{align}
\hbox{for \crc:} \qquad &	\min_{k\in \mathcal{C}_j,k\neq \ell (t)}\hat{\mu}_k(t)-\hat{\mu}_{\ell(t)}(t)\ge G\left(\frac{\sum_{k\in \mathcal{C}_j}N_k(t)\olog j}{T-\sum_{k\notin \mathcal{C}_j}N_k(t) }\right), \label{C}\\
\hbox{for \cra:} \qquad & \frac{\sum_{k\in \mathcal{C}_j,k\neq \ell(t)}\hat{\mu}_k(t)}{j-1}-\hat{\mu}_{\ell(t)}(t)   \ge G\left(\frac{\sum_{k\in \mathcal{C}_j}N_k(t)\olog j}{T-\sum_{k\notin \mathcal{C}_j}N_k(t) }\right),\label{A}
\end{align} 
where $G(\beta)=1/\sqrt{\beta}-1$ for all $\beta\ge 0$. The idea behind (\ref{C}) is to keep the probability of discarding the best arm at most smaller than that of \sr while using less budget. Note that \eqref{A} is easier to achieve than \eqref{C}. \cra is hence more aggressive than \crc, and reduces the set of arms to $\mathcal{C}_2$ faster, but at the expense of a higher risk. After discarding $\ell_3$, \sred will sample the arms in $\mathcal{C}_2$ evenly, and recommend the empirical best arm in $\mathcal{C}_2$ when the budget is exhausted. The pseudo-code of \sred is presented in Algorithm \ref{alg:crc}.  

\begin{algorithm}
	\SetAlgoLined
       {\color{blue} {\bf Input:} $\theta_0\in (0,\frac{1}{\olog K})\cap \QQ$}\\
 	\SetKwProg{Init}{initialization}{}{}
	\Init{}{
		$\mathcal{C}_K\leftarrow [K],\, j\leftarrow K$, sample each arm $k\in [K]$ once,  update $\{N_k(t)\}_{k\in \mathcal{C}_K} $ and $\hat{\bm}(t)$;
	}
        {\color{blue}\For{$t=K+1,\ldots, \lfloor \theta_0 T\rfloor$}{
        sample $A_t\leftarrow \argmin_{k\in \mathcal{C}_{j}} N_k(t)$ {(tie broken arbitrarily)}, update $ \{N_k(t)\}_{k\in \mathcal{C}_j} $ and $\hat{\bm}(t)$;
        }}
	\For{ {\color{blue}$(t=\lfloor \theta_0T\rfloor+1,\ldots, T)$}}{
		$\ell(t) \leftarrow  \argmin_{k\in \mathcal{C}_j}\hat{\mu}_k(t)$ (tie broken arbitrarily);\\
		\uIf{$j>2$, $N_{\ell(t)}(t)>\max_{k\notin\mathcal{C}_j}N_k(t)$, $(\forall k\in \mathcal{C}_j,\,N_{\ell(t)}(t)=N_{k}(t))$,\\
			 and \eqref{C} (resp. \eqref{A}) holds for \crc (resp. \cra)}{
			$\ell_j\leftarrow \ell(t),\,\mathcal{C}_{j-1}\leftarrow \mathcal{C}_j\setminus \{\ell_j\} ,\, j\leftarrow j-1$
		}
		sample $A_t\leftarrow \argmin_{k\in \mathcal{C}_{j}} N_k(t)$ {(tie broken arbitrarily)}, update $ \{N_k(t)\}_{k\in \mathcal{C}_j} $ and $\hat{\bm}(t)$;
	}
	$\ell_2\leftarrow \ell(T)$; return $\hat{\imath}\leftarrow \argmax_{k\in \mathcal{C}_2} \hat{\mu}_k(T) $ {(tie broken arbitrarily)}.
	\captionof{algocf}{\crc and \cra}\label{alg:crc}
\end{algorithm}



\subsection{Analysis of \crc and \cra}\label{sec:anal cr}
As in Section \ref{sec:sr}, $\mu_1>\mu_2\ge\ldots\ge \mu_K$ is assumed wlog and we further define $\mu_{K+1}=0$. We introduce the following instance-specific quantities needed to state our error probability upper bounds. For $ j\in \{2,\ldots, K\}$, define
%\begin{align*}
$$
\psi_j=\frac{j-1}{j}\left(\mu_{1}-\frac{\sum_{k=2}^j\mu_{k}}{j-1}\right)^2,\quad \bpsi_j=\frac{j-1}{j}\left(\mu_1-\frac{\sum_{k=2}^{j-1}\mu_{k}+\mu_{j+1}}{j-1}\right)^2,\quad \zeta_j=\mu_{j}-\mu_{j+1},
$$
$$
\varphi_j=\frac{\sum_{k=1}^j\mu_{k}}{j}-\mu_{j+1},\quad \text{and} \quad \bxi_j=\inf \left\{   \sum_{k=1}^K(\lambda_k-\mu_k)^2: \bl\in \RR^K,\,   \lambda_1\le \min_{k=2,\ldots,j-1,j+1 }\lambda_k  \right\}.
$$%\end{align*}
 Here we remark $\bxi_j\ge \xi_j$ and $\bpsi_j\ge \psi_j$. These inequalities are proven in Proposition \ref{prop:larger C} and Proposition \ref{prop:larger A} in Appendix \ref{app:opt}.

\begin{theorem}\label{thm:crc}
	Let $\bm\in  [0,1]^K$. Under \crc, $\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\imath}\neq 1\right]}$ is larger than
		$$
2\min_{j=2,\ldots,K}\left\{ \frac{\min\left\{\max \left\{ \frac{\xi_j\olog (j+1)(1-\alpha_{j})\mathbbm{1}_{\{j\neq K\}}}{\olog j},\xi_j\right\},  \bar{\xi}_j\right\}}{j\olog K}\right\},
	$$
	where $\alpha_{j}\in \RR$ is the real number such that 
	$	\frac{2\xi_j\left(1-   \alpha_j \right)}{j\olog j}= [(  (1+\zeta_j)\sqrt{\alpha_j }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    )_+]^2. 	
	$
\end{theorem}

\begin{theorem}\label{thm:cra}
Let $\bm\in  [0,1]^K$. Under \cra, $\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\imath}\neq 1\right]}$ is larger than
$$
2\min_{j=2,\ldots,K}\left\{ \frac{\min\{\max \{ \frac{\psi_j\olog (j+1)(1-\alpha_{j}) \mathbbm{1}_{\{j\neq K\}} }{\olog j},\psi_j\},  \bar{\psi}_j\}}{j\olog K}\right\}, 
$$
where $\alpha_{j}\in \RR$ is the real number such that 
$
\frac{\psi_j\left(1-   \alpha_j \right)}{j\olog j}= \frac{j}{j+1}[(  (1+\varphi_j)\sqrt{\alpha_j }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    )_+]^2.$
\end{theorem}

Note that Theorem \ref{thm:crc} implies that \crc enjoys better performance guarantees than \sr, and hence has for now the best known error probability upper bounds.
 
\medskip
\noindent
{\it Proof sketch.} The complete proof of Theorems \ref{thm:crc} and \ref{thm:cra} are given in Appendices \ref{app:crc} and \ref{app:cra}. We sketch that of Theorem \ref{thm:crc}. The proof consists in upper bounding $\mathbb{P}_{\bm}[\ell_j=1]$ for $j\in \{2,\ldots,K\}$. We focus here on the most challenging case where $j\in \{3,\ldots,K-1\}$ (the analysis is simpler when $j=K$, since the only possible allocation is uniform, and when $j=2$, since the only possible round deciding $\ell_2$ is the last round).  

To upper bound $\mathbb{P}_{\bm}[\ell_j=1]$ using Theorem \ref{thm:Varadaham bandits}, we will show that it is enough to study the large deviations of the process $\{\om(\theta T)\}_{T\ge 1}$ for any fixed $\theta \in (0,1]$  and to define a set $\mathcal{S}\subseteq \RR^K$ under which $\ell_j=\ell (\theta T)=1$. We first observe that $\ell_j=\ell(\theta T)$ restricts the possible values of $\om(\theta T)$: 
$
\om(\theta T)\in \mathcal{X}_j:=	\left\{ \xx\in \Sigma : \exists \sigma\in [K]^2\hbox{ s.t. } x_{\sigma (1)}=\ldots=x_{\sigma (j)}>x_{\sigma (j+1)}>\ldots > x_{\sigma (K)}> 0\right\}.
$
 We can hence just derive the LDP satisfied by $\{\om(\theta T)\}_{T\ge 1}$ on $\mathcal{X}_j$. This is done in Appendix \ref{app:allocation}, and we identify by $I_\theta$ a rate function leading to an LDP upper bound. By defining %$\mathcal{X}_{j,i}(\theta)=	\left\{\xx\in \mathcal{X}_j: 	\theta  x_{\sigma (i)}i\olog i> 1-\theta \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\}$, $\forall i\in \{j,\ldots,K\}$.
 \begin{equation*}%\label{eq:yj2}
\mathcal{X}_{j,i}(\theta)=	\left\{\xx\in \mathcal{X}_j: 	\theta  x_{\sigma (i)}i\olog i> 1-\theta \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\},\,\forall i\in \{j,\ldots,K\},
\end{equation*}
 As it is shown in Appendix \ref{subapp:local} that $I_{\theta}(\xx)=\infty$ if $\xx\in \mathcal{X}_{j,i}(\theta)$ for $i\ge j$,
 we may further restrict to  $\mathcal{X}_j\setminus \cup_{i= j}^K\mathcal{X}_{j,i}(\theta)$.

Next, we explain how to apply Theorem \ref{thm:Varadaham bandits} to upper bound $\mathbb{P}_{\bm}[\ell_j=1]$. Let $\mathcal{J}=\{J\subseteq [K]:\left|J\right|=j,1\in J\}$ as defined in Section \ref{sec:sr}. For all $\beta,\theta \in (0,1]$ and $J\in\mathcal{J}$, we introduce the sets 
\begin{align*}
	\mathcal{S}_{J}(\beta)&=\left\{\bl\in \RR^K:\min_{k\in J}\lambda_k-\lambda_1\ge G(\beta)\right\},\\
	\mathcal{Z}_{J}(\theta,\beta)&=\left\{\zz\in \mathcal{X}_j\setminus  \cup_{i= j}^K\mathcal{X}_{j,i}(\theta):(\forall k\in J,\  z_k=\max_{k'\in [K]}z_{k'}),\ \frac{\theta \sum_{k\in J}z_k\olog j   }{1-\theta\sum_{k\notin J}z_{k}}=\beta\right\}.
\end{align*}
Assume that in round $t$, $ \ell_j=\ell(t)=1,\mathcal{C}_j=J$ and let $\sum_{k\notin J}N_k(t)=\tau\le t$ be the number of times arms outside $J$ are pulled. While $\om(t)\notin \mathcal{X}_{j,j}(t/T)$, we have $\beta = \frac{(t-\tau)\olog j}{T-\tau} \in (0,1]$. Using the criteria (\ref{C}), we observe that
\begin{multline*}
 \sum_{t=K+1}^T\sum_{J\in \mathcal{J}}\PP_{\bm}  \left[  \ell_j=\ell(t)=1,\mathcal{C}_j=J ,\om (t)\in \mathcal{X}_j\setminus \cup_{i=j}^K\mathcal{X}_{j,i}(\frac{t}{T})\right]\\
\le \sum_{t=K+1}^T\sum_{J\in \mathcal{J}}\sum_{\tau\le t,\tau\in \NN} \PP_{\bm}  \left[  \hat{\bm}(t)\in \mathcal{S}_{J}(\frac{(t-\tau)\olog j}{T-\tau}),\om (t)\in \mathcal{Z}_{J}(\frac{t}{T},\frac{(t-\tau)\olog j}{T-\tau}) \right]\\
	\le T^2\left|\mathcal{J}\right|\sup_{\theta\in (0,1],\beta \in (0,1] ,J\in\mathcal{J}} \PP_{\bm}\left[  \hat{\bm}(\theta T)\in \mathcal{S}_J(\beta),\om (\theta T)\in \mathcal{Z}_J(\theta,\beta) \right],
\end{multline*}
where the last inequality directly follows from simply upper bounding the number of elements in the sum and from the fact $t\le T$. Hence by applying Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\mathcal{S}_J(\beta)$, $W=\mathcal{Z}_J(\theta,\beta)$ and for any $(\theta,\beta,J)\in (0,1]^2\times {\cal J}$ will lead to an upper bound on $\PP_{\bm}\left[\ell_j=1\right]$. Fix $(\theta,\beta,J)$, Theorem \ref{thm:Varadaham bandits} yields:
$$
\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}( \theta T)\in \mathcal{S}_J(\beta) ,\om (\theta T)\in \mathcal{Z}_J(\theta,\beta)\right]}\ge \theta\inf_{\zz\in \cl(\mathcal{Z}_{J}(\theta,\beta))}\max\{F_{\mathcal{S}_{J}(\beta)}(\zz), I_\theta(\zz)\}.
$$
The proof is completed by providing lower bounds of $\theta F_{S_{J}(\beta)}(\zz)$ and $\theta I_{\theta} (\zz)$ for a fixed $\zz\in \mathcal{Z}_J(\theta,\beta)$ with various $J$. Such bounds are derived in Appendix \ref{app:opt C} and \ref{subapp:rate C}, respectively.
\eproof


\noindent
{\bf Example 2.} To conclude this section, we just illustrate through a simple example the gain in terms of performance guarantees brought by \sred compared to \sr. Assume we have 50 arms with $\mu_1=0.95,\mu_2=0.85,\mu_3=0.2$,  and $\mu_k=0$ for $k=4,\ldots,50$. For \sr, Theorem \ref{thm:sr} states that with a budget of 5000 samples, the error probability of \sr does not exceed $1.93\times 10^{-3}$. With the same budget, Theorems \ref{thm:crc} and \ref{thm:cra} state that the error probabilities of \crc and \cra do not exceed $6.40\times 10^{-4}$ and $6.36\times 10^{-4}$, respectively.
{\color{blue}
\begin{remark}
    In general, we cannot say that one of our two algorithms, \crc or \cra, is better than the other. We illustrate this below for the instances presented in Appendix \ref{num:1} and \ref{num:4}. For the instances in \ref{num:1}, we can easily prove that the performance guarantee for \crc is better than that for \cra. On the contrary, for the instances in \ref{num:4}, \cra has better performance guarantees than \crc. 
\end{remark}}








==> sec/appC_crOLD.tex <==
\section{Analysis of \sred}\label{app_cr}

In \ref{app:crc}, we give the proof for Theorem \ref{thm:crc} and in \ref{app:cra} that of Theorem \ref{thm:cra}. As mentioned in \textsection \ref{sec:sr} and \textsection \ref{sec:anal cr}, in the following analysis, we will assume that $1\ge \mu_1>\mu_2\ge\ldots\ge \mu_K\ge 0$.

\subsection{Performance analysis of \crc}\label{app:crc}
\begin{reptheorem}{thm:crc}
Let $\bm\in  [0,1]^K$. Under \crc, $\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\imath}\neq 1\right]}$ is larger than
$$
2\min_{j=2,\ldots,K}\left\{ \frac{\min\left\{\max \left\{ \frac{\xi_j\olog (j+1)(1-\alpha_{j})\mathbbm{1}_{\{j\neq K\}}}{\olog j},\xi_j\right\},  \bar{\xi}_j\right\}}{j\olog K}\right\},
$$
where $\alpha_{j}\in \RR$ is the real number such that 
$$
 \frac{2\xi_j\left(1-   \alpha_j \right)}{j\olog j}= \left[\left(  (1+\zeta_j)\sqrt{\alpha_j }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2.
$$

\end{reptheorem}
\noindent
We upper bound $\PP_{\bm}\left[\ell_j=1\right]$ for (i) $j=K$; (ii) $j=2$; (iii) $j\in \{3,\ldots,K\}$. The upper bound for (i), presented in \ref{subapp:cK}, is the easiest to derive as the only possible allocation before one discards the first arm is uniform among all arms. The bound for (ii), presented in \ref{subapp:c2}, is the second easiest to derive as $\ell_2$ is decided only in the end, namely, in the $T$-th round. The upper bound for (iii), presented in \ref{subapp:cj}, is more involved since we have to consider all possible allocations and rounds. 
\subsubsection{Upper bound of $\PP_{\bm}\left[\ell_K=1\right]$}\label{subapp:cK}
\begin{lemma}
Let $\bm\in  [0,1]^K$. Under \crc, 
	$$
\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_K= 1\right]}\ge  \frac{2\xi_K}{K\olog K}.
	$$
\end{lemma}
\begin{proof}
Observe that 
\begin{equation}\label{eq:cK 1}
		\PP_{\bm}\left[\ell_K=1\right]= \sum_{t=K+1}^T	\PP_{\bm}\left[\ell_K=\ell(t)=1\right].
\end{equation}
Since \crc discards $\ell_K=\ell(t)$ at the round $t$ only when $N_{\ell(t)}(t)=N_k(t)$ for all $k\in [K]$, it suffices to consider $\om(t)\in \mathcal{X}_K=\{(1/K,\ldots,1/K)\}$. Hence, 
\begin{equation}\label{eq:cK 2}
	 \sum_{t=K+1}^T	\PP_{\bm}\left[\ell_K=\ell(t)=1\right]\le  \sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor}		\PP_{\bm}\left[\ell_K=\ell(t)=1\right]+  \sum_{t= \lfloor \frac{T}{\olog K}\rfloor +1}^T\PP_{\bm}\left[\om (t)\in \mathcal{X}_K\right].
\end{equation}
We upper bound the two terms on the r.h.s. of (\ref{eq:cK 2}) separately. We will prove that the second term in (\ref{eq:cK 2}) is negligible, and restrict our attention to the first term. 

\noindent
\underline{\bf The 2nd term in (\ref{eq:cK 2}).} Notice that 
\begin{equation}\label{eq:cK 3}
	\sum_{t= \lfloor \frac{T}{\olog K}\rfloor +1}^T\PP_{\bm}\left[\om (t)\in \mathcal{X}_K\right]\le T\sup_{\theta \in (1/\olog K,1]} \PP_{\bm}\left[  \om (\theta T)\in \mathcal{X}_K \right].
\end{equation}
And for each $\theta \in (1/\olog K,1]$, we apply Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\RR^K$, $W=\mathcal{X}_K$ to get that
\begin{equation}\label{eq:cK 4}
	\lowlim_{T\rightarrow \infty} \frac{1}{T} \log \frac{1}{ \PP_{\bm}\left[  \om (\theta T)\in \mathcal{X}_K \right]}\ge \inf_{\xx\in\mathcal{X}_K}I_{\theta}(\xx)=\theta  I_{\theta}((1/K,\ldots, 1/K))=\infty,
\end{equation}
where the last equation directly follows from Theorem \ref{thm:crc main rate} with (a) in Appendix \ref{subapp:local}. From (\ref{eq:cK 3})-(\ref{eq:cK 4}), we conclude that we can focus on the first term in (\ref{eq:cK 2}).


\noindent
\underline{\bf The 1st term in (\ref{eq:cK 2}).} Introduce 
$$
\mathcal{S}_{\theta}=\left\{\bl\in \RR^K:\lambda_1\le \min_{k\neq 1}\lambda_k-G(\theta\olog K)\right\},\,\forall \theta\in (0,\frac{1}{\olog K}].
$$
With this notation, we can use the criteria of discarding the arm $\ell_K=\ell(t)=1$ (see \eqref{C}) to get that:
\begin{align}\label{eq:cK 5}
\nonumber	 \sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor}   \PP_{\bm}\left[ \ell_K=\ell(t)=1\right] &\le  \sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor}   \PP_{\bm}\left[ \hat{\bm}(t) \in \mathcal{S}_{\frac{t}{T}},\om (t)\in \mathcal{X}_K  \right]\\
	 &     \le T \sup_{\theta\in (0,1/\olog K ]} \PP_{\bm}\left[   \hat{\bm}(\theta T) \in \mathcal{S}_{\theta},\om (\theta T)\in \mathcal{X}_K        \right].
\end{align}
For each $\theta \in (0,1/\olog K]$, applying (c) in Section \ref{sec:varadaham} with  $\mathcal{S}=\mathcal{S}_\theta$ and $W=\mathcal{X}_K$ yields that  $\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{\theta}, \om (\theta T)\in \mathcal{X}_K\right]}$ is larger than
\begin{align}\label{eq:cK 6}
	\nonumber	\min_{\xx\in\mathcal{X}_K} \theta F_{\mathcal{S}_\theta}(\xx)&=\frac{\theta }{ K}\inf\left\{\sum_{k=1}^K d(\lambda_k,\mu_k):\lambda_1 \le \min_{k\neq 1}\lambda_k-G(\theta \olog K)\right\}\\
	&\ge\frac{2\theta }{K} \inf \left\{ \sum_{k=1}^K (\lambda_k-\mu_k)^2:\lambda_1 \le \min_{k\neq 1}\lambda_k-G(\theta \olog K)\right\} \ge  \frac{2\xi_K}{K\olog K},
\end{align} 
where the first inequality is from Assumption \ref{ass1}, and the last inequality follows from Proposition \ref{prop:crc G} in Appendix \ref{app:opt C} with $\beta=\theta \olog K$. Hence, from (\ref{eq:cK 5})-(\ref{eq:cK 6}), a simple rearrangement yields that
$$
	\lowlim_{T\rightarrow \infty} \frac{1}{T} \log \frac{1}{\sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor} \PP_{\bm}\left[    \ell_K=\ell(t)=1\right]}\ge  \frac{2\xi_K}{K\olog K},
$$
which is also the lower bound for $	\lowlim_{T\rightarrow \infty} \frac{1}{T} \log \frac{1}{\PP_{\bm}\left[\ell_K=1\right]}$ thanks to (\ref{eq:cK 1})-(\ref{eq:cK 2})-(\ref{eq:cK 3})-(\ref{eq:cK 4}).
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	v
%%%%%%%%%%%%%%%%%%%%%%%%	v
%%%%%%%%%%%%%%%%%%%%%%%%	
\subsubsection{Upper bound of $\PP_{\bm}\left[\ell_2=1\right]$}\label{subapp:c2}
\begin{lemma}\label{lem4}
	Let $\bm\in  [0,1]^K$. Under \crc, 
	$$
	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_2= 1\right]}\ge   \frac{\min\{\max \{ 4\xi_2(1-\alpha_2),3\xi_2 \},3\bar{\xi}_2\}}{3\olog K},
	$$
	where $\alpha_2\in \RR$ is the real number such that
	\begin{equation}\label{eq:C alpha 2}
	\xi_2\left(1-   \alpha_2 \right)= \left[\left(  (1+\zeta_2)\sqrt{\alpha_2 }-\frac{1}{2}    \right)_+\right]^2. 	
	\end{equation}
\end{lemma}
\begin{proof}
There are two arms remaining in the last phase. Hence, it suffices to consider the estimate and allocation in the last round. The possible allocation $\om (T)$ belongs to the set
$$
\mathcal{X}_2=\left\{  \xx\in \Sigma: \exists \sigma:[K]  \mapsto [K] \hbox{ s.t. } x_{\sigma (1)}=x_{\sigma (2)}>x_{\sigma (3)}> \ldots > x_{\sigma (K)}> 0\right\}.
$$	
Further introduce for all $i\in \{2,\ldots, K\}$,	
$$
\mathcal{X}_{2,i}(1)=	\left\{\xx\in \mathcal{X}_2: 	x_{\sigma (i)}i\olog i> 1- \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\}.
$$	
We have: 
\begin{equation}\label{eq:c2 1}
	\PP_{\bm}\left[\ell_2=1\right]\le \PP_{\bm}\left[\ell_2=1,\om (T)\in \mathcal{X}_2\setminus \cup_{i= 2}^K\mathcal{X}_{2,i}(1)\right]+\PP_{\bm}\left[\om (T)\in \cup_{i= 2}^K\mathcal{X}_{2,i}(1)\right].
\end{equation}
We will upper bound the two terms in the r.h.s. of (\ref{eq:c2 1}) separately. We will prove that the second term in (\ref{eq:c2 1}) is negligible, and restrict our attention to the first term. 

\medskip
\noindent
\underline{\bf The 2nd term in (\ref{eq:c2 1}).} Note that Theorem \ref{thm:Varadaham bandits}, applied to $\mathcal{S}=\RR^K$, $ W=\cup_{i= 2}^K\mathcal{X}_{2,i}(1)$, implies that
\begin{equation}\label{eq:c2 2}
	\lowlim_{T\rightarrow \infty} \frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \om(T)\in   \cup_{i= 2}^K\mathcal{X}_{2,i}(1) \right]}\ge \inf_{\om \in \cup_{i= 2}^K\mathcal{X}_{2,i}(1) }I_1(\om)=\infty,
\end{equation}
where the equality in (\ref{eq:c2 2}) comes from Theorem \ref{thm:crc main rate} with (a) in Appendix \ref{subapp:local}. As a consequence of (\ref{eq:c2 2}), we can focus on the first term in (\ref{eq:c2 1}).

\medskip
\noindent
\underline{\bf The 1st term in (\ref{eq:c2 1}).} 
As we defined $\mathcal{J}$ in Section \ref{sec:sr}, we introduce $\mathcal{D}=\{D\subseteq [K]:\left|D\right|=2,1\in D\}$, and define for $D\in \mathcal{D}$, 
\begin{align*}
	\mathcal{S}_{D}&=\left\{\bl\in \RR^K:\min_{k\in [D]}\lambda_k\ge \lambda_1\right\},\\	
\text{ and } 	\mathcal{Z}_{D}(1,1)&=\left\{\zz\in   \mathcal{X}_2\setminus \cup_{i= 2}^K\mathcal{X}_{2,1}(1)        :\forall k\in D,\  z_k=\max_{k'\in [K]}z_{k'}\right\}.
\end{align*}
Here the argument $(1,1)$ in $\mathcal{Z}_{D}(1,1)$ is to be consistent with our notation in Appendix \ref{app:allocation}, but we abbreviate it as $\mathcal{Z}_D$ for short below. Since $\ell_2$ is decided as the empirical worst arm in $\mathcal{C}_2$, we can bound the first term in (\ref{eq:c2 1}) as:
\begin{align}\label{eq:c2 3}
\nonumber	\PP_{\bm}\left[\ell_2=1,\om (T)\in \mathcal{X}_2\setminus \cup_{i= 2}^K\mathcal{X}_{2,1}(1)\right]&\le \sum_{D\in \mathcal{D}}   \PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]\\
	&\le (K-1)\sup_{D\in\mathcal{D}} \PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right],
\end{align}
where the last inequality is due to $\left|\mathcal{D}\right|=K-1$. To apply Theorem \ref{thm:Varadaham bandits} on $ \PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]$, we have to analyze $ F_{\mathcal{S}_D}$ and $ I_{1}$ (the  rate function for the process $\{\om ( T)\}_{T\ge 1}$).
For any $\zz\in \mathcal{Z}_{D}$,
\begin{align}\label{eq:c2 4}
		\nonumber	F_{S_{D}}(\zz) &=\inf_{\bl\in \cl(S_D)} \Psi(\bl,\zz)\\
	\nonumber	&\ge 2    \inf\left\{\sum_{k\in D} z_k(\lambda_k-\mu_k)^2:\bl\in \RR^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\}\\
	&\ge  \left(1-\sum_{k\notin D}z_k\right)    \inf\left\{\sum_{k\in D} (\lambda_k-\mu_k)^2:\bl\in \RR^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\},
\end{align}
where the first inequality follows from Assumption \ref{ass1} and the last inequality uses the fact that for $k\in D$, $z_k=(1-\sum_{k'\notin D}z_k')/2$. Next, we consider two cases: (a) $D\neq [2]$; (b) $D=[2]$.

\noindent
\underline{\bf(a) The case where $D\neq [2]$.} Using (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_D$ and $W=\mathcal{Z}_D$, we lower bound the first term in (\ref{eq:c2 1}) as:
\begin{equation}\label{eq:c2 5}
\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]}\ge \inf_{\zz\in \mathcal{Z}_D} F_{\mathcal{S}_{D}}(\zz).
\end{equation}
We then give a lower bound $F_{\mathcal{S}_{D}}(\zz)$ for an arbitrary $\zz \in \mathcal{Z}_D$ by leveraging (\ref{eq:c2 4}). Using Corollary \ref{cor:crc G new} with $\beta =1,j=2$ in Appendix \ref{app:opt C} yields that the r.h.s. of (\ref{eq:c2 4}) is bounded as:
\begin{align}\label{eq:c2 6}
	\nonumber   \left(1-\sum_{k\notin D}z_k\right)    \inf\left\{\sum_{k\in D} (\lambda_k-\mu_k)^2:\bl\in \RR^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\}	&\ge\left(1-\sum_{k\notin D}z_k\right) \bar{\xi}_2\\
	&\ge \frac{\bar{\xi}_2}{\olog K},
\end{align}
where the last inequality directly comes from Proposition \ref{prop ybound} with $\theta =1,\,j=2,\,i=3$ in Appendix \ref{subapp:infinite I}. From (\ref{eq:c2 4})-(\ref{eq:c2 5})-(\ref{eq:c2 6}), we deduce that $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]}\ge\frac{\bar{\xi}_2}{\olog K}$.


\noindent
\underline{\bf (b) The case where $D= [2]$.} Next, we will show that both $\frac{\xi_2}{\olog K}$ and $\frac{4\xi_2(1-\alpha_2)}{3\olog K}$ are lower bounds for $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{[2]},\om (T)\in   \mathcal{Z}_{[2]} \right]}$. The maximum of these hence becomes our lower bound. Together with the conclusion obtained in the case (a), we complete the proof of Lemma \ref{lem4}.


%%%%Some new statement%


%%%%%%
\underline{Lower bounding by $\frac{\xi_2}{\olog K}$.} 
One can, as in the case (a), apply (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_{[2]}$ and $W=\mathcal{Z}_{[2]}$ and (\ref{eq:c2 4}) to obtain that
\begin{align}
\nonumber	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{[2]},\om (T)\in   \mathcal{Z}_{[2]} \right]}&	\ge \inf_{\zz\in \mathcal{Z}_{[2]}} F_{\mathcal{S}_{[2]}}(\zz) \\
\nonumber	  & \ge  \left(1-\sum_{k=3}^K z_k\right)    \inf_{\bl\in \RR^K,\, \lambda_2> \lambda_1}\left\{\sum_{k\in [2]} (\lambda_k-\mu_k)^2\right\}\\
\label{eq:c2 7}& \ge \left(1-\sum_{k=3}^Kz_{\sigma (k)}\right) \xi_2\\
\label{eq:c2 8}&\ge \frac{\xi_2}{\olog K}, 
\end{align}
where the third inequality is derived by Proposition \ref{prop:crc G} with $\theta =1, \beta=1, j=2$ in Appendix \ref{app:opt C}, and the last inequality follows from Proposition \ref{prop ybound} with $j=2,i=3$ in Appendix \ref{subapp:finite I}.\\

\noindent
\underline{Lower bounding by $\frac{4\xi_2(1-\alpha_2)}{3\olog K} $}. Alternatively, one can derive another lower bound by using Theorem \ref{thm:Varadaham bandits} and its rate function for the process $\{\om (T)\}_{T\ge 1}$. In Theorem \ref{thm:crc main rate} with (b), $j=2,\theta=\beta=1$ in Appendix \ref{subapp:local}, we show that 
\begin{equation}\label{eq:c2 9}
 I_{1}(\zz)=\frac{4}{3\olog K}   \left[\left(  (1+\zeta_2)\sqrt{\frac{ z_{\sigma(3)}}{ 1-\sum_{k=4}^Kz_{\sigma(k)}  }}-\frac{1}{2}    \right)_+\right]^2,\,\forall \zz\in \mathcal{Z}_{[2]}
\end{equation}
satisfies LDP upper bound (\ref{eq:rate UB}) for the process $\{\om (T)\}_{T\ge 1}$.

\noindent
Instead of using (\ref{eq:c2 8}), we lower bound $ F_{S_{[2]}}(\zz)$ as:
\begin{align}\label{eq:c2 10}
	\nonumber 	 F_{S_{[2]}}(\zz)&\ge 	 \left(1-\sum_{k=3}^Kz_{\sigma (k)}\right) \xi_2 \\
	\nonumber	&=\xi_2 \left(1- \sum_{k=4}^Kz_{\sigma(k)}  \right) \left(1-   \frac{z_{\sigma(3)}}{1- \sum_{k=4}^Kz_{\sigma(k)} }\right)\\
	&\ge \frac{4\xi_2}{3\olog K} \left(1-   \frac{z_{\sigma(3)}}{1- \sum_{k=4}^Kz_{\sigma(k)} }\right),
\end{align}
where the first inequality follows the derivation of (\ref{eq:c2 7}) and  the last inequality stems from Proposition \ref{prop ybound} with $\theta=1,j=2,i=4$ in Appendix \ref{subapp:finite I}. Since $F_{S_{[2]}}(\zz)$ and $I_{1}(\zz)$ are lower bounded by the functions of $\alpha =  \frac{  z_{\sigma(3)}}{1- \sum_{k=4}^K z_{\sigma (k)}} $ given in  (\ref{eq:c2 9}) and (\ref{eq:c2 10}), applying Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\mathcal{S}_{[2]}$, $W=\mathcal{Z}_{[2]}$ yields that 
\begin{align}\label{eq:c2 11}
\nonumber \lowlim_{T\rightarrow \infty}  \frac{1}{T} & \log \frac{1}{\PP_{\bm}\left[ \hat{\bm}( T)\in\mathcal{S}_{[2]},\om ( T)\in \mathcal{Z}_{[2]}  \right]} \\
\nonumber&\ge \frac{4}{3\olog K} \inf_{\alpha\in \RR} \max\{ \xi_2\left(1-   \alpha \right) ,     [(  (1+\zeta_2)\sqrt{\alpha }-\frac{1}{2}    )_+]^2 \}\\
&\ge  \frac{4\xi_2(1-\alpha_2)}{3\olog K},
\end{align}
where the last inequality is due to Lemma \ref{lem:simple sol new1} in Appendix \ref{app:maxmin} and $\alpha_2$ is defined in (\ref{eq:C alpha 2}). Hence, the maximum of the r.h.s. of (\ref{eq:c2 8}) and (\ref{eq:c2 11}) is a lower bound for $\lowlim_{T\rightarrow \infty}  \frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}( T)\in\mathcal{S}_{[2]},\om ( T)\in \mathcal{Z}_{[2]}  \right]} $.

\noindent
Combining the results for the cases (a) and (b), we conclude that:
$$
\min_{ D\in \mathcal{D}} \lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om ( T)\in \mathcal{Z}_{D} \right]}\ge\frac{\min\{\max \{ \frac{4\xi_2(1-\alpha_2)}{3},\xi_2 \},\bar{\xi}_2 \}}{\olog K} ,
$$ 
which is also a lower bound for  $\lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_2=1 \right]}$ thanks to (\ref{eq:c2 1})-(\ref{eq:c2 2})-(\ref{eq:c2 3}).
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
{\color{blue}
\begin{proof}
    There are two arms remaining in the last phase. Hence, it suffices to consider the estimate and allocation in the last round. The possible allocation $\om (T)$ belongs to the set
$$
\mathcal{X}_2=\left\{  \xx\in \Sigma: \exists \sigma:[K]  \mapsto [K] \hbox{ s.t. } x_{\sigma (1)}=x_{\sigma (2)}>x_{\sigma (3)}> \ldots > x_{\sigma (K)}> 0\right\}.
$$	
As we defined $\mathcal{J}$ in Section \ref{sec:sr}, we introduce $\mathcal{D}=\{D\subseteq [K]:\left|D\right|=2,1\in D\}$. Under this notion, $\mathcal{X}_2=\cup_{D\in \mathcal{D}}{\cal X}_D$, where 
$$
\mathcal{X}_D= \left\{\xx\in {\cal X}_2: \min_{k\in D}x_k>\max_{k'\notin D}x_{k'}\right\}.
$$
Since $\ell_2$ is decided as the empirical worst arm in $\mathcal{C}_2$, 
\begin{align}\label{eq:c121}
 \nonumber \PP_{\bm}[\ell_2=1]&\le \sum_{D\in {\cal D}}\PP_{\bm}[\hat{\bm} (T)\in {\cal S}_D,\om (T)\in {\cal X}_D]\\
 &\le (K-1)\max_{D\in {\cal D}}\PP_{\bm} [\hat{\bm} (T)\in {\cal S}_D,\om (T)\in {\cal X}_D],
\end{align}
where 
$$
\mathcal{S}_{D}=\left\{\bl\in [0,1]^K:\min_{k\in [D]}\lambda_k\ge \lambda_1\right\},
$$
and the last inequality directly follows from counting the number of elements in ${\cal D}$.
Rearranging (\ref{eq:c121}) yields that 
\begin{align}
    \nonumber \lowlim_{T\to \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}[\ell_2=1]} &\ge \lowlim_{T\to\infty}\min_{D\in {\cal D}} \frac{1}{T}\log\frac{1}{\PP_{\bm}[ \hat{\bm} (T)\in {\cal S}_D,\om (T)\in {\cal X}_D]}\\
\nonumber     &\ge \min_{D\in {\cal D}}  \lowlim_{T\to\infty}\frac{1}{T}\log\frac{1}{\PP_{\bm}[ \hat{\bm} (T)\in {\cal S}_D,\om (T)\in {\cal X}_D]} \\
\label{eq:c122}&\ge \min_{D\in {\cal D}} \inf_{\om \in \cl ({\cal X}_D)} \max\{ F_{{\cal S}_{D}}(\om ), I_1(\om )\},
\end{align}
where $I_1$ denotes the rate function for which $\{\om (T)\}_{T\ge 1}$ satisfies an LDP upper bound (\ref{eq:rate UB}), and the second inequality follows from Theorem \ref{thm:Varadaham bandits} with ${\cal S}={\cal S}_D, W={\cal X}_D $.

Further introduce for all $i\in \{2,\ldots, K\}$,	
$$
\mathcal{X}_{2,i}(1)=	\left\{\xx\in \mathcal{X}_2: 	x_{\sigma (i)}i\olog i> 1- \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\}.
$$	
In Theorem \ref{thm:crc main rate} with (a) in Appendix \ref{subapp:local}, we show that $I_1(\om )=\infty$ for all $\om \in \cup_{i=2}^K{\cal X}_{2,i}(1)$, hence any $\om \in \cup_{i=2}^K{\cal X}_{2,i}(1)$ will not be the minimizer on the r.h.s. of (\ref{eq:c122}). In the following, we define 
$$
{\cal Z}_D (1,1)={\cal X}_D\setminus  \cup_{i=2}^K{\cal X}_{2,i}(1).
$$
Here the argument $(1,1)$ in $\mathcal{Z}_{D}(1,1)$ is to be consistent with our notation in Appendix \ref{app:allocation}, but we abbreviate it as $\mathcal{Z}_D$ for short below. For lower bounding (\ref{eq:c122}), we consider two cases: (a) $D\neq [2]$; (b) $D=[2]$.

\noindent
\underline{\bf(a) The case where $D\neq [2]$.} Using Corollary \ref{cor:crc G new} with $\beta =1,j=2$ in Appendix \ref{app:opt C} yields that:
\begin{align}
\nonumber   \inf_{\om \in \cl ({\cal X}_D)} \max\{ F_{{\cal S}_{D}}(\om ), I_1(\om )\}& \ge \inf_{z\in \cl ({\cal Z}_D )}  F_{{\cal S}_{D}}(\zz )\\
\label{eq:c123} &\ge  \left(1-\sum_{k\notin D}z_k\right)    \inf\left\{\sum_{k\in D} (\lambda_k-\mu_k)^2:\bl\in [0,1]^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\}\\	
\nonumber &\ge\left(1-\sum_{k\notin D}z_k\right) \bar{\xi}_2\\
\label{eq:c124}&\ge \frac{\bar{\xi}_2}{\olog K},
\end{align}
where the last inequality directly comes from Proposition \ref{prop ybound} with $\theta =1,\,j=2,\,i=3$ in Appendix \ref{subapp:infinite I}.

%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
\underline{\bf (b) The case where $D= [2]$.} Next, we will show that both $\frac{\xi_2}{\olog K}$ and $\frac{4\xi_2(1-\alpha_2)}{3\olog K}$ are lower bounds for $\inf_{\om \in \cl ({\cal X}_D)} \max\{ F_{{\cal S}_{D}}(\om ), I_1(\om )\}$. The maximum of these hence becomes our lower bound. Together with the conclusion obtained in the case (a), we complete the proof of Lemma \ref{lem4}.


%%%%%%
\underline{Lower bounding by $\frac{\xi_2}{\olog K}$.} 
Observe that (\ref{eq:c123}) holds also for $D=[2]$, hence 
\begin{align}
\nonumber	\inf_{\om \in \cl ({\cal X}_{[2]})} \max\{ F_{{\cal S}_{[2]}}(\om ), I_1(\om )\}&\ge  \inf_{\om \in \cl ({\cal Z}_{[2]})} F_{{\cal S}_{[2]}}(\om ) \\
\nonumber& \ge  \left(1-\sum_{k=3}^K z_k\right)    \inf_{\bl\in \RR^K,\, \lambda_2> \lambda_1}\left\{\sum_{k\in [2]} (\lambda_k-\mu_k)^2\right\}\\
\label{eq:c125}& \ge \left(1-\sum_{k=3}^Kz_{k}\right) \xi_2\\
\label{eq:c126}&\ge \frac{\xi_2}{\olog K}, 
\end{align}
where the second inequality is derived by Proposition \ref{prop:crc G} with $\theta =1, \beta=1, j=2$ in Appendix \ref{app:opt C}, and the last inequality follows from Proposition \ref{prop ybound} with $j=2,i=3$ in Appendix \ref{subapp:finite I}.\\

\underline{Lower bounding by $\frac{4\xi_2(1-\alpha_2)}{3\olog K} $}. One can derive another lower bound by using $I_1$. In Theorem \ref{thm:crc main rate} with (b), $j=2,\theta=\beta=1$ in Appendix \ref{subapp:local}, we show that 
\begin{equation}\label{eq:c127}
 I_{1}(\zz)=\frac{4}{3\olog K}   \left[\left(  (1+\zeta_2)\sqrt{\frac{ z_{\sigma(3)}}{ 1-\sum_{k=4}^Kz_{\sigma(k)}  }}-\frac{1}{2}    \right)_+\right]^2,\,\forall \zz\in \mathcal{Z}_{[2]}
\end{equation}
is a valid rate function for an LDP upper bound (\ref{eq:rate UB}) for the process $\{\om (T)\}_{T\ge 1}$.

\noindent
Instead of using (\ref{eq:c126}), we lower bound $ F_{S_{[2]}}(\zz)$ as:
\begin{align}\label{eq:c128}
	\nonumber 	 F_{S_{[2]}}(\zz)&\ge 	 \left(1-\sum_{k=3}^Kz_{\sigma (k)}\right) \xi_2 \\
	\nonumber	&=\xi_2 \left(1- \sum_{k=4}^Kz_{\sigma(k)}  \right) \left(1-   \frac{z_{\sigma(3)}}{1- \sum_{k=4}^Kz_{\sigma(k)} }\right)\\
	&\ge \frac{4\xi_2}{3\olog K} \left(1-   \frac{z_{\sigma(3)}}{1- \sum_{k=4}^Kz_{\sigma(k)} }\right),
\end{align}
where the first inequality follows the derivation of (\ref{eq:c125}) and the last inequality stems from Proposition~\ref{prop ybound} with $\theta=1,j=2,i=4$ in Appendix~\ref{subapp:finite I}. Since $F_{S_{[2]}}(\zz)$ and $I_{1}(\zz)$ are lower bounded by the functions of $\alpha =  \frac{  z_{\sigma(3)}}{1- \sum_{k=4}^K z_{\sigma (k)}} $ given in (\ref{eq:c127}) and (\ref{eq:c128}), applying Theorem~\ref{thm:Varadaham bandits} with $\mathcal{S}=\mathcal{S}_{[2]}$, $W=\mathcal{Z}_{[2]}$ yields that 
\begin{align}\label{eq:c129}
\nonumber\inf_{\om \in \cl ({\cal X}_{[2]})} \max\{ F_{{\cal S}_{[2]}}(\om ), I_1(\om )&\ge \frac{4}{3\olog K}  \inf_{\alpha\in \RR} \max\{ \xi_2\left(1-   \alpha \right) ,     [(  (1+\zeta_2)\sqrt{\alpha }-\frac{1}{2}    )_+]^2 \}\\
&\ge  \frac{4\xi_2(1-\alpha_2)}{3\olog K},
\end{align}
where the last inequality is due to Lemma \ref{lem:simple sol new1} in Appendix \ref{app:maxmin} and $\alpha_2$ is defined in (\ref{eq:C alpha 2}). Hence, the maximum of the r.h.s. of (\ref{eq:c126}) and (\ref{eq:c129}) is a lower bound for $\lowlim_{T\rightarrow \infty}  \frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}( T)\in\mathcal{S}_{[2]},\om ( T)\in \mathcal{Z}_{[2]}  \right]} $.


\end{proof}}
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Upper bound for $\PP_{\bm}\left[\ell_j=1\right]$ for $j\in \{3,\ldots,K-1\}$}\label{subapp:cj}
\begin{lemma}\label{lem5}
	Let $\bm\in  [0,1]^K,\,j\in \{3,\ldots,K-1\}  $. Under \crc, 
	$$
	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_j= 1\right]}\ge    \frac{2\min\left\{\max \left\{ \frac{\xi_j\olog (j+1)(1-\alpha_{j})}{\olog j},\xi_j\right\},  \bar{\xi}_j\right\}}{j\olog K},
$$
	where $\alpha_j\in \RR$ is the real number such that
\begin{equation}\label{eq:C alpha j}
	 \frac{2\xi_j\left(1-   \alpha_j \right)}{j\olog j}= \left[\left(  (1+\zeta_j)\sqrt{\alpha_j }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2. 	
\end{equation}
\end{lemma}

\begin{proof}
Observe that 
\begin{equation}\label{eq:cj 1}
\PP_{\bm}\left[\ell_j=1\right]= \sum_{t=K+1}^{T} \PP_{\bm}\left[\ell_j=\ell(t)=1\right].	
\end{equation}
In round $t$, $\ell_j$ is discarded only when there are $j$ arm remaining, $N_{\ell (t)}(t)>\max_{k\notin \mathcal{C}_j}N_k(t)$, and $ N_k(t)=N_{k'}(t)$ for all $k\in \mathcal{C}_j$. Hence, we only need to consider the scenario where $\om(t)\in \mathcal{X}_j$, where
$$
	\mathcal{X}_j=\left\{ \xx\in \Sigma : \exists \sigma: [K] \mapsto [K] \hbox{ s.t. } x_{\sigma (1)}=\ldots=x_{\sigma (j)}>x_{\sigma (j+1)}> \ldots > x_{\sigma (K)}> 0\right\}.
$$ 
Further introducing for any $\theta\in (0,1],\,i\in \{j,\ldots, K\}$,
$$
	\mathcal{X}_{j,i}(\theta)=	\left\{\xx\in \mathcal{X}_j: 	\theta  x_{\sigma (i)}i\olog i> 1-\theta \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\},
$$
 we simply get that (\ref{eq:cj 1}) is smaller than
 \begin{equation}\label{eq:cj 2}
   \sum_{t=K+1}^{T} \PP_{\bm}\left[\ell_j=\ell(t)=1,\om (t)\in \mathcal{X}_j\setminus \cup_{i= j}^K\mathcal{X}_{j,i}(\frac{t}{T}) \right]+  \sum_{t=K+1}^{T} \PP_{\bm}\left[  \om(t)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\frac{t}{T})\right].		 	
 \end{equation}
 We will prove that the second term in (\ref{eq:cj 2}) is negligible, and restrict our attention to the first term. 
 
\underline{\bf The 2nd term in (\ref{eq:cj 2}).} Observe that
 \begin{equation}\label{eq:cj 3}
 	  \sum_{t=K+1}^{T} \PP_{\bm}\left[  \om(t)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\frac{t}{T})\right] \le T\sup_{\theta\in (0,1]} \PP_{\bm}\left[  \om(\theta T)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\theta )\right]
 \end{equation}
 and for each $\theta \in (0,1]$, Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\RR^K$ and $W= \cup_{i= j}^K\mathcal{X}_{j,i}(\theta )$ implies that
 \begin{equation}\label{eq:cj 4}
 	\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{ \PP_{\bm}\left[  \om(\theta T)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\theta )\right]}\ge\theta \inf_{\xx\in\cup_{i=j}^K\mathcal{X}_{j,i}(\theta)}I_{\theta}(\xx)=\infty,
 \end{equation}
where the equality follows directly from Theorem \ref{thm:crc main rate} with (a) in Appendix \ref{subapp:local}. From (\ref{eq:cj 3}) and (\ref{eq:cj 4}), one can focus on the first term in (\ref{eq:cj 2}). 

\medskip
\noindent
\underline{\bf The 1st term in (\ref{eq:cj 2}).} Suppose that in round $t$, $\mathcal{C}_j=J$ for some $J\in\mathcal{J}$, and let $\sum_{k\notin J}N_k(t)=\tau\le t$ be the number of times arms outside $J$ are pulled. While $\ell_j=\ell(t)=1$, we must have $\hat{\bm}(t)\in \mathcal{S}_{J}(\frac{(t-\tau)\olog j}{T-\tau})$, where 
 $$
 \mathcal{S}_J(\beta)=\left\{ \bl\in \RR^K:\min_{k\in J}\lambda_k-\lambda_1\ge G(\beta)   \right\},\,\forall \beta \in (0,1],
 $$
 because $\frac{(t-\tau)\olog j}{T-\tau}=\frac{\sum_{k\in\mathcal{C}_j}N_k(t)\olog j  }{T-\sum_{k\notin \mathcal{C}_j}N_k(t) }$ (recall the discarding condition (\ref{C})). Notice if $\om (t)\notin \mathcal{X}_{j,j}(\frac{t}{T})\subseteq \cup_{i=j}^K \mathcal{X}_{j,i}(\frac{t}{T})$, it directly follows that $\frac{(t-\tau)\olog j}{T-\tau}\le 1$. Now further introduce 
 $$
 \mathcal{Z}_{J}(\theta,\beta)=\left\{\zz\in \mathcal{X}_j\setminus  \cup_{i= j}^K\mathcal{X}_{j,i}(\theta):(\forall k\in J,\  z_k=\max_{k'\in [K]}z_{k'}),\ \frac{\theta \sum_{k\in J}z_k\olog j   }{1-\theta\sum_{k\notin J}z_{k}}=\beta\right\},
 $$
 $\forall \theta,\beta\in (0,1]$. These allow us to upper bound the first term in (\ref{eq:cj 2}) by
 \begin{align}\label{eq:cj 5}
\nonumber  \sum_{t=K+1}^T\sum_{J\in \mathcal{J}}\sum_{\tau\le t}\PP_{\bm}\left[\hat{\bm}(t)\in \mathcal{S}_J(\frac{(t-\tau)\olog j}{T-\tau}),\om (t)\in \mathcal{Z}_J(\frac{t}{T}, \frac{(t-\tau)\olog j}{T-\tau} )\right]\\
 	\le \left|\mathcal{J}\right|T^2\sup_{\beta,\theta\in (0,1]}\PP_{\bm}\left[\hat{\bm}(\theta T)\in \mathcal{S}_J(\beta),\om(\theta T)\in \mathcal{Z}_J(\theta,\beta)\right],
 \end{align}
 where the last inequality follows from simply upper bounding the number of elements in the sum. To apply Theorem \ref{thm:Varadaham bandits}, we have to analyze $F_{\mathcal{S}_J(\beta)}$ and $I_{\theta}$ ($I_{\theta}$ is the rate function for the process $\{\om (\theta T)\}_{T\ge 1}$). If $\zz\in\mathcal{Z}_{J}(\theta,\beta)$,
 \begin{align}\label{eq:cj 6}
 	\nonumber	\theta F_{S_{J}(\beta)}(\zz) &=\theta\inf_{\bl\in \cl(S_J(\beta))} \Psi(\bl,\zz)\\
 	\nonumber												&\ge 2\inf\left\{\sum_{k\in J}\theta z_k(\lambda_k-\mu_k)^2:\min_{k\in J,k\neq 1}\lambda_k-\lambda_1\ge G(\beta)\right\}\\
 										&= \frac{2}{j\olog j}\left(1-\theta \sum_{k\notin J}z_k\right)\beta\inf\left\{\sum_{k\in J}(\lambda_k-\mu_k)^2:\min_{k\in J,k\neq 1}\lambda_k-\lambda_1\ge G(\beta)\right\},
 \end{align}
 where the first inequality is due to Assumption \ref{ass1}; the second equality uses the fact that $\forall k\in J,\, \theta z_k =\frac{(1-\theta\sum_{k'\notin J}z_{k'})\beta}{j\olog j}$ (as $\zz\in\mathcal{Z}_J(\theta,\beta)$). Next we consider two cases: (a) $J\neq [j]$ and (b) $J=[j]$.\\

 \noindent
\underline{\bf (a) The case where $J\neq [j]$.} We invoke Corollary \ref{cor:crc G new} in Appendix \ref{app:opt C} to lower bound the r.h.s. of (\ref{eq:cj 6}) by 
 $$
 	 \frac{2\bar{\xi}_j}{j\olog j}(1-\theta \sum_{k\notin J}z_k)   \ge \frac{2\bar{\xi}_j}{j\olog K},
 $$
 where the inequality is a consequence of Proposition \ref{prop ybound} with $i=j+1$ in Appendix \ref{subapp:finite I}. Applying (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_J(\beta)$, $W=\mathcal{Z}_J(\theta,\beta)$ yields that
 \begin{equation}
 	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{J}(\theta,\beta),\om (\theta T)\in \mathcal{Z}_J(\theta,\beta)  \right]} \ge\inf_{\zz\in \mathcal{Z}_{J}(\theta,\beta)} \theta F_{S_{J}(\beta)}(\zz)\ge \frac{2\bar{\xi}_j}{j\olog K}.
 \end{equation}
\underline{\bf (b) The case where $J=[j]$.} We will show that both $\frac{2\xi_j}{j\olog K}$ and $\frac{2\xi_j\olog (j+1)(1-\alpha_j)}{j\olog j\olog K}$ are lower bounds for $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{[j]}(\beta),\om (\theta T)\in \mathcal{Z}_{[j]}(\theta,\beta)  \right]} $. The maximum of these becomes our lower bound. Together with the conclusion obtained in the case (a), we complete the proof of Lemma \ref{lem5}.


%%%%%%
\underline{Lower bounding by $\frac{2\xi_j}{j\olog K}$}.
%%%%%%%%%
By Proposition \ref{prop:crc G} and Proposition \ref{prop ybound}, we can further lower bound the r.h.s. of (\ref{eq:cj 6}) as
\begin{align}
\nonumber	\theta F_{S_{J}(\beta)}(\zz) & \ge \frac{2}{j\olog j}\left(1-\theta \sum_{k\notin J}z_k\right)\beta\inf\left\{\sum_{k\in J}(\lambda_k-\mu_k)^2:\min_{k\in J,k\neq 1}\lambda_k-\lambda_1\ge G(\beta)\right\}\\
\label{eq:cj 7}	&\ge 	\frac{2\xi_j}{j\olog j}\left(1-\theta \sum_{k\notin J}z_k\right)\\
\label{eq:cj 8}	& \ge \frac{2\xi_j}{j\olog K},
\end{align}
where the first inequality corresponds to (\ref{eq:cj 6}); the second inequality is due to Proposition \ref{prop:crc G} in Appendix \ref{app:opt C}; the last inequality uses Proposition \ref{prop ybound} with $i=j+1$ in  Appendix \ref{subapp:finite I}.

\noindent
Then one can, as in the case (a), apply (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_{[j]}(\beta)$, $W=\mathcal{Z}_{[j]}(\theta,\beta)$ and (\ref{eq:cj 8}) to obtain that 
  \begin{equation}\label{eq:cj 9}
 	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{[j]}(\beta),\om (\theta T)\in \mathcal{Z}_{[j]}(\theta,\beta)  \right]} \ge\inf_{\zz\in \mathcal{Z}_{[j]}(\theta,\beta)} \theta F_{S_{[j]}(\beta)}(\zz)\ge \frac{2\xi_j}{j\olog K}.
 \end{equation}
\noindent
\underline{Lower bounding by $\frac{2\xi_j\olog (j+1)(1-\alpha_j)}{j\olog j\olog K}$}. Alternatively, one can lower bound the l.h.s. of (\ref{eq:cj 9}) by using Theorem \ref{thm:Varadaham bandits} and its rate function for the process $\{\om (\theta T)\}_{T\ge 1}$. In Theorem \ref{thm:crc main rate} with (b) in Appendix \ref{subapp:local}, we shows that 
 \begin{equation}\label{eq:cj 10}
\theta I_{\theta}(\zz)=\frac{\olog (j+1)}{\olog K}   \left[\left(  (1+\zeta_j)\sqrt{\frac{\theta z_{\sigma(j+1)}}{ 1-\theta\sum_{k=j+2}^Kz_{\sigma(k)}  }}-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2,
 \end{equation}
 $\,\forall \zz\in \mathcal{Z}_{[j]}(\theta,\beta)$, satisfies an LDP upper bound (\ref{eq:rate UB}) for the process $\{\om (\theta T)\}_{T\ge 1}$.


\noindent
Instead of (\ref{eq:cj 8}), we lower bound $\theta F_{S_{[j]}(\beta)}(\zz)$ as:
 \begin{align}\label{eq:cj 11}
\nonumber 	\theta F_{S_{[j]}(\beta)}(\zz)\ge \frac{2\xi_j}{j\olog j}\left(1-\theta \sum_{k\notin [j]}z_k\right)	 &=\frac{2\xi_j}{j\olog j} \left(1-\theta \sum_{k=j+2}^Kz_{\sigma(k)}  \right) \left(1-   \frac{\theta z_{\sigma(j+1)}}{1-\theta \sum_{k=j+2}^Kz_{\sigma(k)} }\right)\\
 	 &\ge \frac{2\xi_j\olog (j+1)}{j\olog j\olog K} \left(1-   \frac{\theta z_{\sigma(j+1)}}{1-\theta \sum_{k=j+2}^Kz_{\sigma(k)} }\right),
 \end{align}
 where the first inequality is from (\ref{eq:cj 7}) and the last inequality is due to Proposition \ref{prop ybound} with $i=j+2$ in Appendix \ref{subapp:finite I}. Since $\theta F_{S_{[j]}(\beta)}(\zz)$ and $\theta I_{\theta}(\zz)$ are lower bounded by the functions of $\alpha =  \frac{ \theta z_{\sigma(j+1)}}{1-\theta \sum_{k=j+2}^K z_{\sigma (k)}} $ given in (\ref{eq:cj 10}) and (\ref{eq:cj 11}), applying Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\mathcal{S}_{[j]}(\beta)$, $W=\mathcal{Z}_{[j]}(\theta,\beta)$ yields that
 \begin{multline}\label{eq:cj 12}
\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in\mathcal{S}_{[j]}(\beta),\om (\theta T)\in \mathcal{Z}_{[j]}(\theta,\beta)  \right]} \ge\\
\frac{\olog (j+1)}{\olog K} \inf_{\alpha\in \RR} \max\left\{ \frac{2\xi_j\left(1-   \alpha \right)}{j\olog j} ,     \left[\left(  (1+\zeta_j)\sqrt{\alpha }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2 \right\}.
 \end{multline}
 By Lemma \ref{lem:simple sol new1} in Appendix \ref{app:maxmin}, (\ref{eq:cj 12}) is lower bounded by $\frac{2\xi_j\olog (j+1)(1-\alpha_j)}{j\olog j\olog K}$, where $\alpha_j$ is described in (\ref{eq:C alpha j}).
Combining (a) and (b), we conclude that 
\begin{multline*}
\min_{ J\in \mathcal{J}}\inf_{\beta,\theta\in (0,1]} \lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\bm}(\theta T)\in \mathcal{S}_{J}(\beta),\om (\theta T)\in \mathcal{Z}_J(\theta,\beta)  \right]}\ge \\
    \frac{2\min\{\max \{ \frac{\xi_j\olog (j+1)(1-\alpha_{j})}{\olog j},\xi_j\},  \bar{\xi}_j\}}{j\olog K},	
\end{multline*}
which is also a lower bound for $\lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_j=1 \right]}$ thanks to (\ref{eq:cj 1})-(\ref{eq:cj 2})-(\ref{eq:cj 3})-(\ref{eq:cj 4}).
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Performance analysis of \cra}\label{app:cra}
\begin{reptheorem}{thm:cra}
	Let $\bm\in  [0,1]^K$. Under \cra, $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\imath}\neq 1\right]}$ is larger than
	$$
	2\min_{j=2,\ldots,K}\left\{ \frac{\min\{\max \{ \frac{\psi_j\olog (j+1)(1-\alpha_{j}) \mathbbm{1}_{\{j\neq K\}} }{\olog j},\psi_j\},  \bar{\psi}_j\}}{j\olog K}\right\},  
	$$
	where $\alpha_{j}\in \RR$ is the real number such that 
	$$
		\frac{\psi_j\left(1-   \alpha_j \right)}{j\olog j}= \frac{j}{j+1}\left[\left(  (1+\varphi_j)\sqrt{\alpha_j }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2.
	$$
\end{reptheorem}
We upper bound $\PP_{\bm}\left[\ell_j=1\right]$ for (i) $j=K$; (ii) $j=2$; (iii) $j\in \{3,\ldots,K\}$. The upper bound for (i), presented in \ref{subapp:aK}, is the easiest to derive as the only possible allocation before one discards the first arm is uniform among all arms. The bound for (ii), presented in \ref{subapp:a2}, is the second easiest to derive as $\ell_2$ is decided only in the end, namely, in the $T$-th round. The upper bound for (iii), presented in \ref{subapp:aj}, is more involved since we have to consider all possible allocations and rounds. 

%%%%%%%%%%%%
\subsubsection{Upper bound of $\PP_{\bm}\left[\ell_K=1\right]$}\label{subapp:aK}
\begin{lemma}
	Let $\bm\in  [0,1]^K$. Under \cra, 
	$$
	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_K= 1\right]}\ge  \frac{2\psi_K}{K\olog K}.
	$$
\end{lemma}
\begin{proof}
	Observe that 
	\begin{equation}\label{eq:aK 1}
		\PP_{\bm}\left[\ell_K=1\right]= \sum_{t=K+1}^T	\PP_{\bm}\left[\ell_K=\ell(t)=1\right].
	\end{equation}
	Since \cra discards $\ell_K=\ell(t)$ in round $t$ only when $N_{\ell(t)}(t)=N_k(t)$ for all $k\in [K]$, it suffices to consider $\om(t)\in \mathcal{X}_K=\{(1/K,\ldots,1/K)\}$. Hence
	\begin{equation}\label{eq:aK 2}
		\sum_{t=K+1}^T	\PP_{\bm}\left[\ell_K=\ell(t)=1\right]\le  \sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor}		\PP_{\bm}\left[\ell_K=\ell(t)=1\right]+  \sum_{t= \lfloor \frac{T}{\olog K}\rfloor +1}^T\PP_{\bm}\left[\om (t)\in \mathcal{X}_K\right].
	\end{equation}
	We upper bound the two terms on the r.h.s. of (\ref{eq:aK 2}) separately. We will prove that the second term in (\ref{eq:aK 2}) is negligible, and restrict our attention to the first term. 
	
	\noindent
	\underline{\bf The 2nd term in (\ref{eq:aK 2}).} Notice that 
	\begin{equation}\label{eq:aK 3}
		\sum_{t= \lfloor \frac{T}{\olog K}\rfloor +1}^T\PP_{\bm}\left[\om (t)\in \mathcal{X}_K\right]\le T\sup_{\theta \in (1/\olog K,1]} \PP_{\bm}\left[  \om (\theta T)\in \mathcal{X}_K \right].
	\end{equation}
	And for each $\theta \in (1/\olog K,1]$, we apply Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\RR^K$, $W=\mathcal{X}_K$ to get that
	\begin{equation}\label{eq:aK 4}
		\lowlim_{T\rightarrow \infty} \frac{1}{T} \log \frac{1}{ \PP_{\bm}\left[  \om (\theta T)\in \mathcal{X}_K \right]}\ge \inf_{\xx\in\mathcal{X}_K}I_{\theta}(\xx)=\theta  I_{\theta}((1/K,\ldots, 1/K))=\infty,
	\end{equation}
	where the last equality directly follows from Theorem \ref{thm:cra main rate} with (a) in Appendix \ref{subapp:local}. From (\ref{eq:aK 3})-(\ref{eq:aK 4}), we conclude that we can focus on the first term in (\ref{eq:aK 2}).
	
	
	\noindent
	\underline{\bf The 1st term in (\ref{eq:aK 2}).} Introduce 
	$$
	\mathcal{S}_{\theta}=\left\{\bl\in \RR^K:\lambda_1\le \frac{\sum_{k=2}^K\lambda_k}{K-1}-G(\theta\olog K)\right\},\,\forall \theta\in (0,\frac{1}{\olog K}].
	$$
	With this notation, we can use the criteria of discarding the arm $\ell_K=\ell(t)=1$ (see \eqref{A}) to get that:
	\begin{align}\label{eq:aK 5}
		\nonumber	 \sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor}   \PP_{\bm}\left[ \ell_K=\ell(t)=1\right] &\le  \sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor}   \PP_{\bm}\left[ \hat{\bm}(t) \in \mathcal{S}_{\frac{t}{T}},\om (t)\in \mathcal{X}_K  \right]\\
		&     \le T \sup_{\theta\in (0,1/\olog K ]} \PP_{\bm}\left[   \hat{\bm}(\theta T) \in \mathcal{S}_{\theta},\om (\theta T)\in \mathcal{X}_K        \right].
	\end{align}
	For each $\theta \in (0,1/\olog K]$, applying (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_\theta$ and $W=\mathcal{X}_K$ yields that  $\lowlim_{T\rightarrow}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{\theta}, \om (\theta T)\in \mathcal{X}_K\right]}$ is larger than
	\begin{align}\label{eq:aK 6}
		\nonumber	\min_{\xx\in\mathcal{X}_K} \theta F_{\mathcal{S}_\theta}(\xx)&=\frac{\theta }{ K}\inf\left\{\sum_{k=1}^K d(\lambda_k,\mu_k):\lambda_1 \le  \frac{\sum_{k=2}^K\lambda_k}{K-1}-G(\theta \olog K)\right\}\\
		&\ge\frac{2\theta }{K} \inf \left\{ \sum_{k=1}^K (\lambda_k-\mu_k)^2:\lambda_1 \le  \frac{\sum_{k=2}^K\lambda_k}{K-1}-G(\theta \olog K)\right\} \ge  \frac{2\psi_K}{K\olog K},
	\end{align} 
	where the first inequality is from Assumption \ref{ass1}, and the last inequality follows from Proposition \ref{prop:cra G} in Appendix \ref{app:opt A} with $\beta=\theta \olog K$. Hence, from (\ref{eq:aK 5})-(\ref{eq:aK 6}), a simple rearrangement yields that
	$$
	\lowlim_{T\rightarrow \infty} \frac{1}{T} \log \frac{1}{\sum_{t=K+1}^{\lfloor \frac{T}{\olog K}\rfloor} \PP_{\bm}\left[    \ell_K=\ell(t)=1\right]}\ge  \frac{2\psi_K}{K\olog K},
	$$
	which is also the lower bound for $	\lowlim_{T\rightarrow \infty} \frac{1}{T} \log \frac{1}{\PP_{\bm}\left[\ell_K=1\right]}$ thanks to (\ref{eq:aK 1})-(\ref{eq:aK 2})-(\ref{eq:aK 3})-(\ref{eq:aK 4}).
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
\subsubsection{Upper bound of $\PP_{\bm}\left[\ell_2=1\right]$}\label{subapp:a2}
\begin{lemma}\label{lem7}
	Let $\bm\in  [0,1]^K$. Under \cra, 
	$$
	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_2= 1\right]}\ge   \frac{\min\{\max \{ 4\psi_2(1-\alpha_2),3\psi_2 \},3\bar{\psi}_2\}}{3\olog K},
	$$
	where $\alpha_2\in \RR$ is the real number such that
	\begin{equation}\label{eq:A alpha 2}
		3\psi_2\left(1-   \alpha_2 \right)= 4\left[\left(  (1+\varphi_2)\sqrt{\alpha_2 }-\frac{1}{2}    \right)_+\right]^2. 	
	\end{equation}
\end{lemma}
\begin{proof}
	As there are two arms remaining in the last phase, it suffices to study the estimate and the allocation in the last round. The possible allocation, $\om (T)$ belongs to the set
	$$
	\mathcal{X}_2=\left\{  \xx\in \Sigma: \exists \sigma:[K]  \mapsto [K] \hbox{ s.t. } x_{\sigma (1)}=x_{\sigma (2)}>x_{\sigma (3)}> \ldots > x_{\sigma (K)}> 0\right\}.
	$$	
	Further introduce for all $i\in \{2,\ldots, K\}$,	
	$$
	\mathcal{X}_{2,i}(1)=	\left\{\xx\in \mathcal{X}_2: 	x_{\sigma (i)}i\olog i> 1- \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\}.
	$$	
	We get that 
	\begin{equation}\label{eq:a2 1}
		\PP_{\bm}\left[\ell_2=1\right]\le \PP_{\bm}\left[\ell_2=1,\om (T)\in \mathcal{X}_2\setminus \cup_{i= 2}^K\mathcal{X}_{2,i}(1)\right]+\PP_{\bm}\left[\om (T)\in \cup_{i= 2}^K\mathcal{X}_{2,i}(1)\right],
	\end{equation}
	and we will bound two terms in the r.h.s. of (\ref{eq:a2 1}) separately. We will prove that the second term in (\ref{eq:c2 1}) is negligible, and restrict our attention to the first term. 
	
	\medskip
	\noindent
	\underline{\bf The 2nd term in (\ref{eq:a2 1}).} Note that Theorem \ref{thm:Varadaham bandits}, applied to $\mathcal{S}=\RR^K$, $ W=\cup_{i= 2}^K\mathcal{X}_{2,1}(1)$, implies 
	\begin{equation}\label{eq:a2 2}
		\lowlim_{T\rightarrow \infty} \frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \om(T)\in   \cup_{i= 2}^K\mathcal{X}_{2,i}(1) \right]}\ge \inf_{\om \in \cup_{i= 2}^K\mathcal{X}_{2,i}(1) }I_1(\om)=\infty,
	\end{equation}
	where the equality in (\ref{eq:a2 2}) comes Theorem \ref{thm:cra main rate} with (b), $j=2,\theta=\beta=1$ in Appendix \ref{subapp:local}. As a consequence of (\ref{eq:a2 2}), we can focus on the first term in (\ref{eq:a2 1}).
	
	\medskip
	\noindent
	\underline{\bf The 1st term in (\ref{eq:a2 1}).} 
	As we defined $\mathcal{J}$ in Section \ref{sec:sr}, we introduce $\mathcal{D}=\{D\subseteq [K]:\left|D\right|=2,1\in D\}$, and define for $D\in \mathcal{D}$,
	\begin{align*}
		\mathcal{S}_{D}&=\left\{\bl\in \RR^K:\min_{k\in [D]}\lambda_k\ge \lambda_1\right\},\\	
		\text{ and } 	\mathcal{Z}_{D}(1,1)&=\left\{\zz\in   \mathcal{X}_2\setminus \cup_{i= 2}^K\mathcal{X}_{2,1}(1)          :\forall k\in D,\  z_k=\max_{k'\in [K]}z_{k'}\right\}.
	\end{align*}
	Here the argument $(1,1)$ in $\mathcal{Z}_{D}(1,1)$ is to be consistent with our notation in Appendix \ref{app:allocation}, but we abbreviate it as $\mathcal{Z}_D$ for short below. Since $\ell_2$ is decided as the empirical worst arm in $\mathcal{C}_2$, we can bound the first term in (\ref{eq:a2 1}) as:
	\begin{align}\label{eq:a2 3}
		\nonumber	\PP_{\bm}\left[\ell_2=1,\om (T)\in \mathcal{X}_2\setminus \cup_{i= 2}^K\mathcal{X}_{2,1}(1)\right]&\le \sum_{D\in \mathcal{D}}   \PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]\\
		&\le (K-1)\sup_{D\in\mathcal{D}} \PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right],
	\end{align}
	where the last inequality is due to $\left|\mathcal{D}\right|=K-1$. To apply Theorem \ref{thm:Varadaham bandits} on $ \PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]$, we  have to analyze $ F_{\mathcal{S}_D}$ and $ I_{1}$ (the  rate function for the process $\{\om ( T)\}_{T\ge 1}$).
	For any $\zz\in \mathcal{Z}_{D}$,
	\begin{align}\label{eq:a2 4}
		\nonumber	F_{S_{D}}(\zz) &=\inf_{\bl\in \cl(S_D)} \Psi(\bl,\om)\\
		\nonumber	&\ge 2    \inf\left\{\sum_{k\in D} z_k(\lambda_k-\mu_k)^2:\bl\in \RR^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\}\\
		&\ge  \left(1-\sum_{k\notin D}z_k\right)    \inf\left\{\sum_{k\in D} (\lambda_k-\mu_k)^2:\bl\in \RR^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\},
	\end{align}
	where the first inequality follows from Assumption \ref{ass1} and the last one uses the fact that for $k\in D$, $z_k=(1-\sum_{k'\notin D}z_k')/2$. Next, we consider two cases: (a) $D\neq [2]$; (b) $D=[2]$.
	
	\noindent
	\underline{\bf(a) The case where $D\neq [2]$.} Using (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_D$ and $W=\mathcal{Z}_D$, we lower bound the first term in (\ref{eq:a2 1}) as:
	\begin{equation}\label{eq:a2 5}
		\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]}\ge \inf_{\zz\in \mathcal{Z}_D} F_{\mathcal{S}_{D}}(\zz).
	\end{equation}
	We then give a lower bound of $F_{\mathcal{S}_{D}}(\zz)$ for an arbitrary $\zz \in \mathcal{Z}_D$ by leveraging (\ref{eq:a2 4}). Using Corollary \ref{cor:cra G new} with $\beta =1,j=2$ in Appendix \ref{app:opt A} yields that the r.h.s. of (\ref{eq:a2 4}) is bounded as:
	\begin{align}\label{eq:a2 6}
		\nonumber   \left(1-\sum_{k\notin D}z_k\right)    \inf\left\{\sum_{k\in D} (\lambda_k-\mu_k)^2:\bl\in \RR^K,\,\min_{k\in D}\lambda_k= \lambda_1\right\}	&\ge\left(1-\sum_{k\notin D}z_k\right) \bar{\psi}_2\\
		&\ge \frac{\bar{\psi}_2}{\olog K},
	\end{align}
	where the last inequality directly comes from Proposition \ref{prop ybound} with $\theta =1,\,j=2,\,i=3$ in Appendix \ref{subapp:infinite I}. From (\ref{eq:a2 4})-(\ref{eq:a2 5})-(\ref{eq:a2 6}), we deduce that $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{D},\om (T)\in   \mathcal{Z}_{D} \right]}\ge\frac{\bar{\psi}_2}{\olog K}$.
	
	
	\noindent
	\underline{\bf (b) The case where $D= [2]$.} 
 Next, we will show that both $\frac{\psi_2}{\olog K}$ and $ \frac{4\psi_2(1-\alpha_2)}{3\olog K}$ are lower bounds for $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{[2]},\om (T)\in   \mathcal{Z}_{[2]} \right]}$. The maximum of these hence becomes our lower bound. Together with the conclusion obtained in the case (a), we complete the proof of Lemma \ref{lem7}.
 
 %%%%%%
 \underline{Lower bounding by $ \frac{\xi_2}{\olog K}$.} One can, as in the case (a), apply (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_{[2]}$ and $W=\mathcal{Z}_{[2]}$ and (\ref{eq:a2 4}) to obtain that
	\begin{align}
		\nonumber	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(T)\in \mathcal{S}_{[2]},\om (T)\in   \mathcal{Z}_{[2]} \right]}&	\ge \inf_{\zz\in \mathcal{Z}_{[2]}} F_{\mathcal{S}_{[2]}}(\zz) \\
		\nonumber	  & \ge  \left(1-\sum_{k=3}^K z_k\right)    \inf_{\bl\in \RR^K,\, \lambda_2> \lambda_1}\left\{\sum_{k\in [2]} (\lambda_k-\mu_k)^2\right\}\\
		\label{eq:a2 7}& \ge \left(1-\sum_{k=3}^Kz_{\sigma (k)}\right) \psi_2\\
		\label{eq:a2 8}&\ge \frac{\psi_2}{\olog K}, 
	\end{align}
	where the third inequality is derived by Proposition \ref{prop:cra G} with $\theta =1, \beta=1, j=2$ in Appendix \ref{app:opt A}, and the last inequality follows from Proposition \ref{prop ybound} with $j=2,i=3$ in Appendix \ref{subapp:finite I}.\\
	
	\noindent
\underline{Lower bounding by $\frac{4\psi_2(1-\alpha_2)}{3\olog K} $.} Alternatively, one can derive another lower bound by using Theorem \ref{thm:Varadaham bandits} and the rate function for the process $\{\om (T)\}_{T\ge 1}$. In Theorem \ref{thm:cra main rate} with (b), $j=2,\theta=\beta=1$ in Appendix \ref{subapp:local}, we show that 
\begin{equation}\label{eq:a2 9}
		I_{1}(\zz)=\frac{16}{9\olog K}   \left[\left(  (1+\varphi_2)\sqrt{\frac{ z_{\sigma(3)}}{ 1-\sum_{k=4}^Kz_{\sigma(k)}  }}-\frac{1}{2}    \right)_+\right]^2,\,\forall \zz\in \mathcal{Z}_{[2]}
	\end{equation}
satisfies an LDP upper bound (\ref{eq:rate UB}) for the process $\{\om (T)\}_{T\ge 1}$.

	\noindent
	Instead of using (\ref{eq:a2 8}), we lower bound $ F_{S_{[2]}}(\zz)$ as:
	\begin{align}\label{eq:a2 10}
		\nonumber 	 F_{S_{[2]}}(\zz)&\ge 	 \left(1-\sum_{k=3}^Kz_{\sigma (k)}\right) \psi_2 \\
		\nonumber	&=\psi_2 \left(1- \sum_{k=4}^Kz_{\sigma(k)}  \right) \left(1-   \frac{z_{\sigma(3)}}{1- \sum_{k=4}^Kz_{\sigma(k)} }\right)\\
		&\ge \frac{4\psi_2}{3\olog K} \left(1-   \frac{z_{\sigma(3)}}{1- \sum_{k=4}^Kz_{\sigma(k)} }\right),
	\end{align}
	where the first inequality follows from the derivation of (\ref{eq:a2 7}) and the last inequality stems from Proposition \ref{prop ybound} with $\theta=1,j=2,i=4$ in Appendix \ref{subapp:finite I}. Since $F_{S_{[2]}}(\zz)$ and $I_{1}(\zz)$ are lower bounded by the functions of $\alpha =  \frac{  z_{\sigma(3)}}{1- \sum_{k=4}^K z_{\sigma (k)}} $ given in (\ref{eq:a2 9}) and (\ref{eq:a2 10}), applying Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\mathcal{S}_{[2]}$, $W=\mathcal{Z}_{[2]}$ yields that 
	\begin{align}\label{eq:a2 11}
		\nonumber \lowlim_{T\rightarrow \infty}  \frac{1}{T} &\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}( T)\in\mathcal{S}_{[2]},\om ( T)\in \mathcal{Z}_{[2]}  \right]}\\
  \nonumber&\ge \frac{4}{3\olog K} \inf_{\alpha\in \RR} \max\left\{ \psi_2\left(1-   \alpha \right) ,     \frac{4[(  (1+\varphi_2)\sqrt{\alpha }-\frac{1}{2}    )_+]^2}{3} \right\}\\
		&\ge  \frac{4\psi_2(1-\alpha_2)}{3\olog K},
	\end{align}
	where the last inequality is due to Lemma \ref{lem:simple sol new1} in Appendix \ref{app:maxmin} and $\alpha_2$ is defined in (\ref{eq:A alpha 2}). Hence, the maximum of the r.h.s. of (\ref{eq:a2 8}) and (\ref{eq:a2 11}) is a lower bound for $\lowlim_{T\rightarrow \infty}  \frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}( T)\in\mathcal{S}_{[2]},\om ( T)\in \mathcal{Z}_{[2]}  \right]} $.
	
	\noindent
	Combining the results for the cases (a) and (b), we conclude that:
	$$
	\min_{ D\in \mathcal{D}} \lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\bm}(T)\in \mathcal{S}_{D},\om ( T)\in \mathcal{Z}_{D} \right]}\ge \frac{\min\{\max \{ \frac{4\psi_2(1-\alpha_2)}{3},\psi_2 \},\bar{\psi}_2 \}}{\olog K} ,
	$$ 
	which is also a lower bound for  $\lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_2=1 \right]}$ thanks to (\ref{eq:a2 1})-(\ref{eq:a2 2})-(\ref{eq:a2 3}).
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	
%%%%%%%%%%%%%%%%%%%%%%%%	v

\subsubsection{Upper bound for $\PP_{\bm}\left[\ell_j=1\right]$ for $j\in \{3,\ldots,K-1\}$}\label{subapp:aj}
\begin{lemma}\label{lem8}
	Let $\bm\in  [0,1]^K,\,j\in \{3,\ldots,K-1\}  $. Under \cra, 
	$$
	\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_j= 1\right]}\ge     \frac{2\min\left\{\max \left\{ \frac{\psi_j\olog (j+1)(1-\alpha_{j})}{\olog j},\psi_j\right\},  \bar{\psi}_j\right\}}{j\olog K},	
	$$
	where $\alpha_j\in \RR$ is the real number such that
	\begin{equation}\label{eq:A alpha j}
		\frac{\psi_j\left(1-   \alpha_j \right)}{j\olog j}= \frac{j}{j+1}\left[\left(  (1+\varphi_j)\sqrt{\alpha_j }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2. 	
	\end{equation}
\end{lemma}

\begin{proof}
	Observe that 
	\begin{equation}\label{eq:aj 1}
	\PP_{\bm}\left[\ell_j=1\right]= \sum_{t=K+1}^{T} \PP_{\bm}\left[\ell_j=\ell(t)=1\right].	
	\end{equation}
	In round $t$, $\ell_j$ is discarded only when there are $j$ arm remaining, $N_{\ell (t)}(t)>\max_{k\notin \mathcal{C}_j}N_k(t)$, and $ N_k(t)=N_{k'}(t)$ for all $k\in \mathcal{C}_j$. Hence we only need to consider the allocation $\om (t)\in \mathcal{X}_j$, where
	$$
	\mathcal{X}_j=\left\{ \xx\in \Sigma : \exists \sigma: [K] \mapsto [K] \hbox{ s.t. } x_{\sigma (1)}=\ldots=x_{\sigma (j)}>x_{\sigma (j+1)}> \ldots > x_{\sigma (K)}> 0\right\}.
	$$ 
	Further introducing for all $\theta\in (0,1],\,i\in \{j,\ldots, K\}$,
	$$
	\mathcal{X}_{j,i}(\theta)=	\left\{\xx\in \mathcal{X}_j: 	\theta  x_{\sigma (i)}i\olog i> 1-\theta \sum_{k=i+1}^Kx_{\sigma(k)}	   \right\},
	$$
	we simply get that (\ref{eq:aj 1}) is smaller than
	\begin{equation}\label{eq:aj 2}
		\sum_{t=K+1}^{T} \PP_{\bm}\left[\ell_j=\ell(t)=1,\om (t)\in \mathcal{X}_j\setminus \cup_{i= j}^K\mathcal{X}_{j,i}(\frac{t}{T}) \right]+  \sum_{t=K+1}^{T} \PP_{\bm}\left[  \om(t)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\frac{t}{T})\right].		 	
	\end{equation}
  We will prove that the second term in (\ref{eq:aj 2}) is negligible, and restrict our attention to the first term. 
 
	\underline{\bf The 2nd term in (\ref{eq:aj 2}).} Observe that
	\begin{equation}\label{eq:aj 3}
		\sum_{t=K+1}^{T} \PP_{\bm}\left[  \om(t)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\frac{t}{T})\right] \le T\sup_{\theta\in (0,1]} \PP_{\bm}\left[  \om(\theta T)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\theta )\right]
	\end{equation}
	and for each $\theta \in (0,1]$, Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\RR^K$ and $W= \cup_{i= j}^K\mathcal{X}_{j,i}(\theta )$ implies that
	\begin{equation}\label{eq:aj 4}
\lowlim_{T\rightarrow\infty}\frac{1}{T}\log \frac{1}{ \PP_{\bm}\left[  \om(\theta T)\in \cup_{i= j}^K\mathcal{X}_{j,i}(\theta )\right]}\ge\theta \inf_{\xx\in\cup_{i=j}^K\mathcal{X}_{j,i}(\theta)}I_{\theta}(\xx)=\infty,
	\end{equation}
	where the equality follows directly from Theorem \ref{thm:cra main rate} with (a) in Appendix \ref{subapp:local}. From (\ref{eq:aj 3}) and (\ref{eq:aj 4}), one can focus on the first term in (\ref{eq:aj 2}). 
 
 \medskip
 \noindent
	\underline{\bf The 1st term in (\ref{eq:aj 2}).} Suppose that in round $t$, $\mathcal{C}_j=J$ for some $J\in\mathcal{J}$, and let $\sum_{k\notin J}N_k(t)=\tau\le t$ be the number of times arms outside $J$ are pulled. While $\ell_j=\ell(t)=1$, we must have $\hat{\bm}(t)\in \mathcal{S}_{J}(\frac{(t-\tau)\olog j}{T-\tau})$, where 
	$$
	\mathcal{S}_J(\beta)=\left\{ \bl\in \RR^K: \frac{\sum_{k\in J,k\neq 1}\lambda_k}{j-1}-\lambda_1\ge G(\beta)   \right\},\,\forall \beta \in (0,1],
	$$
	because $\frac{(t-\tau)\olog j}{T-\tau}=\frac{\sum_{k\in\mathcal{C}_j}N_k(t)\olog j   }{T-\sum_{k\notin \mathcal{C}_j}N_k(t) }$ (recall the discarding condition (\ref{A})). Notice if $\om (t)\notin \mathcal{X}_{j,j}(\frac{t}{T})\subseteq \cup_{i=j}^K\mathcal{X}_{j,i}(\frac{t}{T})$, it directly follows that $\frac{(t-\tau)\olog j}{T-\tau}\le 1$. Now further introduce 
	 $$
 \mathcal{Z}_{J}(\theta,\beta)=\left\{\zz\in \mathcal{X}_j\setminus  \cup_{i= j}^K\mathcal{X}_{j,i}(\theta):(\forall k\in J,\  z_k=\max_{k'\in [K]}z_{k'}),\ \frac{\theta \sum_{k\in J}z_k\olog j   }{1-\theta\sum_{k\notin J}z_{k}}=\beta\right\},
 $$
 $\forall \theta,\beta\in (0,1]$. These allow us to upper bound the first term in (\ref{eq:aj 2}) by
	\begin{align}\label{eq:aj 5}
		\nonumber  \sum_{t=K+1}^T\sum_{J\in \mathcal{J}}\sum_{\tau\le t}\PP_{\bm}\left[\hat{\bm}(t)\in \mathcal{S}_J(\frac{(t-\tau)\olog j}{T-\tau}),\om (t)\in \mathcal{Z}_J(\frac{t}{T}, \frac{(t-\tau)\olog j}{T-\tau} )\right]\\
		\le \left|\mathcal{J}\right|T^2\sup_{\beta,\theta\in (0,1]}\PP_{\bm}\left[\hat{\bm}(\theta T)\in \mathcal{S}_J(\beta),\om(\theta T)\in \mathcal{Z}_J(\theta,\beta)\right],
	\end{align}
	where the last inequality follows from simply upper bounding the number of elements in the sum. To apply Theorem \ref{thm:Varadaham bandits}, we have to analyze $F_{\mathcal{S}_J(\beta)}$ and $I_{\theta}$ ($I_{\theta}$ is the rate function for the process $\{\om (\theta T)\}_{T\ge 1}$). If $\zz\in\mathcal{Z}_{J}(\theta,\beta)$,
	\begin{align}\label{eq:aj 6}
		\nonumber	\theta F_{S_{J}(\beta)}(\zz) &=\theta\inf_{\bl\in \cl(S_J(\beta))} \Psi(\bl,\zz)\\
		\nonumber												&\ge 2\inf\left\{\sum_{k\in J}\theta z_k(\lambda_k-\mu_k)^2: \frac{\sum_{k\in J,k\neq 1}\lambda_k}{j-1}-\lambda_1\ge G(\beta)\right\}\\
		&= \frac{2}{j\olog j}\left(1-\theta \sum_{k\notin J}z_k\right)\beta\inf\left\{\sum_{k\in J}(\lambda_k-\mu_k)^2: \frac{\sum_{k\in J,k\neq 1}\lambda_k}{j-1}-\lambda_1\ge G(\beta)\right\},
	\end{align}
	where the first inequality is due to Assumption \ref{ass1}; the second equality uses the fact that $\forall k\in J,\, \theta z_k =\frac{(1-\theta\sum_{k'\notin J}z_{k'})\beta}{j\olog j}$ (as $\zz\in\mathcal{Z}_J(\theta,\beta)$). Next we consider two cases: (a) $J\neq [j]$ and (b) $J=[j]$.\\
	
	 \noindent
	\underline{\bf (a) The case where $J\neq [j]$.} We invoke Corollary \ref{cor:cra G new} in Appendix \ref{app:opt A} to lower bound the r.h.s. of (\ref{eq:aj 6}) by 
	$$
		\frac{2\bar{\psi}_j}{j\olog j}(1-\theta \sum_{k\notin J}z_k)   \ge \frac{2\bar{\psi}_j}{j\olog K},
	$$
	where the inequality is a consequence of Proposition \ref{prop ybound} with $i=j+1$ in Appendix \ref{subapp:finite I}. Applying (c) in Section \ref{sec:varadaham} with $\mathcal{S}=\mathcal{S}_J(\beta)$, $W=\mathcal{Z}_J(\theta,\beta)$ yields that
	$$
		\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{J}(\theta,\beta),\om (\theta T)\in \mathcal{Z}_J(\theta,\beta)  \right]} \ge\inf_{\zz\in \mathcal{Z}_{J}(\theta,\beta)} \theta F_{S_{J}(\beta)}(\zz)\ge \frac{2\bar{\psi}_j}{j\olog K}.
	$$
	\underline{\bf (b) The case where $J=[j]$.} We will show that both $\frac{2\psi_j}{j\olog K}$ and $\frac{2\psi_j\olog (j+1)(1-\alpha_j)}{j\olog j\olog K}$ are lower bounds for $\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{[j]}(\beta),\om (\theta T)\in \mathcal{Z}_{[j]}(\theta,\beta)  \right]} $. The maximum of these becomes our lower bound. Together with the conclusion obtained in the case (a), we then complete the proof of Lemma \ref{lem8}.
 
 %%%%%%%%%%%%%%%%%
 \underline{Lower bounding $\frac{2\psi_j}{j\olog K}$}. By Proposition \ref{prop:cra G} and Proposition \ref{prop ybound}, we can further lower bound the r.h.s. of (\ref{eq:aj 6}) as
	\begin{align}
		\nonumber	\theta F_{S_{J}(\beta)}(\zz) & \ge \frac{2}{j\olog j}\left(1-\theta \sum_{k\notin J}z_k\right)\beta\inf\left\{\sum_{k\in J}(\lambda_k-\mu_k)^2:  \frac{\sum_{k\in J,k\neq 1}\lambda_k}{j-1}  -\lambda_1\ge G(\beta)\right\}\\
		\label{eq:aj 7}	&\ge 	\frac{2\psi_j}{j\olog j}\left(1-\theta \sum_{k\notin J}z_k\right)\\
		\label{eq:aj 8}	& \ge \frac{2\psi_j}{j\olog K},
	\end{align}
	where the first inequality corresponds to (\ref{eq:aj 6}); the second inequality is due to Proposition \ref{prop:cra G} in Appendix \ref{app:opt A}; the last inequality uses Proposition \ref{prop ybound} with $i=j+1$ in  Appendix \ref{subapp:finite I}.
	
	\noindent
	Then one can, as in the case (a), apply (c) in Section \ref{sec:varadaham} $\mathcal{S}=\mathcal{S}_{[j]}(\beta)$, $W=\mathcal{Z}_{[j]}(\theta,\beta)$ and (\ref{eq:aj 8}) to obtain that 
	\begin{equation}\label{eq:aj 9}
		\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in \mathcal{S}_{[j]}(\beta),\om (\theta T)\in \mathcal{Z}_{[j]}(\theta,\beta)  \right]} \ge\inf_{\zz\in \mathcal{Z}_{[j]}(\theta,\beta)} \theta F_{S_{[j]}(\beta)}(\zz)\ge \frac{2\psi_j}{j\olog K}.
	\end{equation}

\underline{Lower bounding by $\frac{2\psi_j\olog (j+1)(1-\alpha_j)}{j\olog j\olog K}$}. Alternatively, one can lower bound the l.h.s. of (\ref{eq:aj 9}) by using Theorem \ref{thm:Varadaham bandits} and its rate function for the process $\{\om (\theta T)\}_{T\ge 1}$. In Theorem \ref{thm:cra main rate} with (b) in Appendix \ref{subapp:local}, we shows that 
\begin{equation}\label{eq:aj 10}
		\theta I_{\theta}(\zz)=\frac{2j\olog (j+1)}{(j+1)\olog K} \left[\left(  (1+\varphi_j)\sqrt{\frac{\theta z_{\sigma(j+1)}}{ 1-\theta\sum_{k=j+2}^Kz_{\sigma(k)}  }}-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2,
	\end{equation} 
 $\,\forall \zz\in \mathcal{Z}_{[j]}(\theta,\beta)$, 
satisfies an LDP upper bound (\ref{eq:rate UB}) for the process $\{\om (\theta T)\}_{T\ge 1}$.


 
\noindent
Instead of (\ref{eq:aj 8}), we lower bound $\theta F_{S_{[j]}(\beta)}(\zz)$ as:
	\begin{align}\label{eq:aj 11}
		\nonumber 	\theta F_{S_{[j]}(\beta)}(\zz)\ge \frac{2\psi_j}{j\olog j}\left(1-\theta \sum_{k\notin [j]}z_k\right)	 &=\frac{2\psi_j}{j\olog j} \left(1-\theta \sum_{k=j+2}^Kz_{\sigma(k)}  \right) \left(1-   \frac{\theta z_{\sigma(j+1)}}{1-\theta \sum_{k=j+2}^Kz_{\sigma(k)} }\right)\\
		&\ge \frac{2\psi_j\olog (j+1)}{j\olog j\olog K} \left(1-   \frac{\theta z_{\sigma(j+1)}}{1-\theta \sum_{k=j+2}^Kz_{\sigma(k)} }\right),
	\end{align}
	where the first inequality is from (\ref{eq:aj 7}) and the last inequality is due to Proposition \ref{prop ybound} with $i=j+2$ in Appendix \ref{subapp:finite I}. Since $\theta F_{S_{[j]}(\beta)}(\zz)$ and $\theta I_{\theta}(\zz)$ are lower bounded by the functions of $\alpha =  \frac{ \theta z_{\sigma(j+1)}}{1-\theta \sum_{k=j+2}^K z_{\sigma (k)}} $ given in (\ref{eq:aj 10}) and (\ref{eq:aj 11}), applying Theorem \ref{thm:Varadaham bandits} with $\mathcal{S}=\mathcal{S}_{[j]}(\beta)$, $W=\mathcal{Z}_{[j]}(\theta,\beta)$ yields that
	\begin{multline}\label{eq:aj 12}
		\lowlim_{T\rightarrow \infty}\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[ \hat{\bm}(\theta T)\in\mathcal{S}_{[j]}(\beta),\om (\theta T)\in \mathcal{Z}_{[j]}(\theta,\beta)  \right]} \ge\\
		\frac{2\olog (j+1)}{\olog K} \inf_{\alpha\in \RR} \max\left\{ \frac{\psi_j\left(1-   \alpha \right)}{j\olog j} ,    \frac{j}{j+1} \left[\left(  (1+\varphi_j)\sqrt{\alpha }-\sqrt{\frac{1}{(j+1)\olog (j+1)}}    \right)_+\right]^2 \right\}.
	\end{multline}
	By Lemma \ref{lem:simple sol new1} in Appendix \ref{app:maxmin}, (\ref{eq:aj 12}) is lower bounded by $\frac{2\psi_j\olog (j+1)(1-\alpha_j)}{j\olog j\olog K}$, where $\alpha_j$ is described in (\ref{eq:A alpha j}).
	Combining the cases (a) and (b), we conclude that 
	\begin{multline*}
		\min_{ J\in \mathcal{J}}\inf_{\beta,\theta\in (0,1]} \lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\hat{\bm}(\theta T)\in \mathcal{S}_{J}(\beta),\om (\theta T)\in \mathcal{Z}_J(\theta,\beta)  \right]}\ge \\
		\frac{2\min\{\max \{ \frac{\psi_j\olog (j+1)(1-\alpha_{j})}{\olog j},\psi_j\},  \bar{\psi}_j\}}{j\olog K},	
	\end{multline*}
	which is also a lower bound for $\lowlim_{T\rightarrow \infty }\frac{1}{T}\log \frac{1}{\PP_{\bm}\left[\ell_j=1 \right]}$ thanks to (\ref{eq:aj 1})-(\ref{eq:aj 2})-(\ref{eq:aj 3})-(\ref{eq:aj 4}).
		%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%
\end{proof}








